Optimal Statistical Inference for Individualized Treatment Effects in High-dimensional Models

The ability to predict individualized treatment effects (ITEs) based on a given patient's profile is essential for personalized medicine. We propose a hypothesis testing approach to choosing between two potential treatments for a given individual in the framework of high-dimensional linear models. The methodological novelty lies in the construction of a debiased estimator of the ITE and establishment of its asymptotic normality uniformly for an arbitrary future high-dimensional observation, while the existing methods can only handle certain specific forms of observations. We introduce a testing procedure with the type-I error controlled and establish its asymptotic power. The proposed method can be extended to making inference for general linear contrasts, including both the average treatment effect and outcome prediction. We introduce the optimality framework for hypothesis testing from both the minimaxity and adaptivity perspectives and establish the optimality of the proposed procedure. An extension to high-dimensional approximate linear models is also considered. The finite sample performance of the procedure is demonstrated in simulation studies and further illustrated through an analysis of electronic health records data from patients with rheumatoid arthritis.

==> Optimality.tex <==
%!TEX root = ITE-Revision.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Optimality for Hypothesis Testing}
\label{sec: optimality}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%{\blue Tony, we have two options of presenting the optimality results. Let $k_1$ denote the true sparsity level and $k_2$ denote the prior knowledge of sparsity level. If no additional information is available, we put $k_2=p$. 
%\begin{enumerate}
%\item We only consider the case where the sparsity level is unknown, that is, $k_2=p$.
%\item We consider the results for different levels of $k_2$ and there is a transition at $k_2=\sqrt{p}$. This case is more general and also more results need to be included. 
%\end{enumerate}
%Although the second is more general, the main concern is that we need to construct optimal confidence interval for arbitrary $k_2$. If $k_2\leq \sqrt{p}$, the construction is different from our paper's method and requires the knowledge of $k_2$, as in our paper \citet{cai2015regci}.
%}

%We define the following null parameter space 
%\begin{equation}
%\HH_0^{G}(k,s)=\HH_0^{G}(k,s,\xi)=\left\{\theta \in \Theta^{G}\left(k,s\right): \xi^{\intercal}\left(\beta-\gamma\right)\leq 0\right\}.
%\end{equation}
%\begin{equation}
%\HH_1^{G}(k,s,\tau)=\left\{\theta \in \Theta^{G}\left(k,s\right): \xi^{\intercal}\left(\beta-\gamma\right)> \tau\right\}. 
%\end{equation}
%The following theorem shows that the proposed testing procedure controls the size and attains a large power under certain sparsity condition.
%\begin{Proposition} 
%\label{prop: general unknown Sigma}
%Suppose that $n\gg \min\{k, \left(\|\xi\|_1/\|\xi\|_2\right)^2 \}(s\log p)^2$, then we have
%\begin{equation}
%\limsup_{n,p\rightarrow \infty} \sup_{\theta\in \HH_0^{G}(k,s)} \E_{\theta} \phi^{*}_{G} \leq \alpha. %quad \text{and} \quad \limsup_{n,p\rightarrow \infty} \sup_{\theta\in \HH_0(s)} \E_{\theta} \phi^{*}_{T}(k) \leq \alpha.
%%\alphab(k,\xi,\phi^{*}_{L})\leq \alpha \quad \text{and} \quad \alphab(k,\xi,\phi^{*}_{T}(k))\leq \alpha.
%\label{eq: unknown Sigma}
%\end{equation}
%For $\tau\gtrsim \frac{\|\xi\|_2}{\sqrt{n}}$, the testing procedure $\phi^{*}_{G}$ defined in \eqref{eq: linear test semi} satisfies 
%\begin{equation}
%\inf_{\theta\in \HH_1^{G}(k,s,\tau)} \E_{\theta}\phi^{*}_{G} \rightarrow 1.
%\end{equation}
%\end{Proposition}
%



In this section, we investigate the optimality of the proposed procedure in the hypothesis testing framework from two perspectives, minimaxity and adaptivity. We introduce the optimality framework  in Section \ref{sec: framework}, present the detailed  results in Section \ref{sec: results}, and compare with the optimality of confidence intervals in Section \ref{sec: comparison}.

%To start with, we assume the sparsity level $k$ to be known a priori and establish the optimality of the hypothesis testing problem in this case. This will be referred to as the minimaxity framework. After this, we also discuss the adaptivity problem for the hypothesis testing \eqref{eq: testing problem}, that is, what will happen if the sparsity level $k$ is unknown. 
%This motivates us to consider the optimality under the adaptivity framework. That is, what is the optimal procedure when the true sparsity is unknown? 
%The optimality from the perspective of minimaxity is established in Section \ref{sec: minimaxity optimality} while that from the perspective of adaptivity is established in Section \ref{eq: adaptivity optimality}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Optimality from the perspective of minimaxity}
%\label{sec: minimaxity optimality}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%We consider the following parameter space for $\left(\beta,\Sigma,\sigma_1,\gamma,\Gamma,\sigma_2\right)$
%\begin{equation}
%\Theta\left(k\right)=\left\{\left(\beta, \Sigma,\sigma_1,\gamma, \Gamma,\sigma_2\right): \max\{\|\beta\|_0,\|\gamma\|_0\}\leq k, 0<\sigma_1,\sigma_2\leq M \right\}.
%\label{eq: signal para space}
%\end{equation}
%For a given sparsity level $k$, we define the null parameter space, 
%\begin{equation}
%\HH_0(s)=\left\{\theta=\left(\beta, \Sigma,\sigma_1,\gamma, \Gamma,\sigma_2\right) \in \Theta(k): \xi^{\intercal}\left(\beta-\gamma\right)\leq 0\right\}
%\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Optimality Framework for  Hypothesis Testing: Minimaxity and Adaptivity}
\label{sec: framework}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The performance of a testing procedure can be evaluated in terms of its size (type I error probability) and its power (or type II error probability). For a given test $\phi$ and a null parameter space $\HH_0(s)$,  its size is
\begin{equation}
{\alphab}(s,\phi)=\sup_{\theta\in \HH_0(s)} \E_{\theta} \phi. 
\label{eq: type I error}
\end{equation}
It has been shown in Corollary \ref{Cor: hypothesis testing} that the proposed test $\phi_{\alpha}$ satisfies ${\alphab}(s,\phi_{\alpha})\leq \alpha.$ %It remains to study what is the best power we can aim for if the proposed procedure controls type I error as in \eqref{eq: type I error}.
%the optimality in terms of the power of the hypothesis testing procedure. %When the parameter $\theta$ is close to (but not belonging to) $\HH_0(s)$, any testing procedure will suffer from a lower power. 
To investigate the power, we consider the following local alternative parameter space %of $\HH_0(s),$
%To investigate the power of the testing procedure, we rule out part of the parameter space close to the null parameter space, $\HH_0(s)$ and introduce the following alternative parameter space, 
%Specifically, ,  we define
$
\HH_1(s,\tau)=\left\{\theta \in \Theta(s):\bx_{\rm new}^{\intercal}\left(\bbeta_1-\bbeta_2\right)=\tau\right\}, 
$
for a given $\tau>0$.
%{eq: null space}
%$\HH_1(s,\tau)$ is the intersection of the parameter space $\Theta\left(k\right)$ and the subspace $\xi^{\intercal}\left(\beta-\gamma\right)> \tau$. 
The power of a test $\phi$ over the parameter space $\HH_1(s,\tau)$ is 
 \begin{equation}
\omegab(s,\tau,\phi)=\inf_{\theta\in \HH_1(s,\tau)} \E_{\theta}\phi.
\label{eq: power definition}
\end{equation}
With a larger value of $\tau$, the alternative parameter space is further away from the null parameter space and hence it is easier to construct a test of higher power. The minimax optimality can be reduced to identifying the smallest $\tau$ such that the size is controlled over $\HH_0(s)$ and the corresponding power over $\HH_1(s,\tau)$ is large, that is,
\begin{equation}
\taumini=\argmin_{\tau}\left\{\tau: \sup_{\phi: \alphab(s,\phi)\leq \alpha}\omegab(s,\tau,\phi)\geq 1-\eta\right\},
\label{eq: detection boundary minimaxity}
\end{equation}
%{\red How about changing $\rightarrow 1-\eta$ to $\ge 1-\eta$?}
where $\eta\in[0,1)$ is a small positive constant controlling the type II error probability. The quantity $\taumini$ depends on $\bx_{\rm new}$, the sparsity level $\kt$ and the constants $\alpha,\eta\in(0,1)$. Throughout the discussion, we omit $\alpha$ and $\eta$ in the arguments of $\taumini$ for simplicity. 
This quantity $\taumini$ is referred to as the minimax detection boundary of the hypothesis testing problem \eqref{eq: testing problem}. In other words, $\taumini$ is the minimum distance such that there exists a test controlling size and achieving a good power. If a test $\phi$ satisfies the following property, %for the testing problem \eqref{eq: testing problem},
\begin{equation}
\alphab(s,\phi)\leq \alpha \quad \text{and} \quad \omegab(s, \phi,\tau)\geq 1-\eta \quad \text{for}\;\; \tau \asymp \taumini
\label{eq: minimax optimal}
\end{equation}
then $\phi$ is defined to be minimax optimal. The minimax detection boundary in \eqref{eq: detection boundary minimaxity} is defined for a given sparsity level $s$, which is assumed to be known a priori. However, the exact sparsity level is typically unknown in practice. Hence, it is also of great importance to consider the optimality from the following two perspectives on adaptivity, 
\begin{enumerate}
\item[Q1.] Whether it is possible to construct a test achieving the minimax detection boundary defined in \eqref{eq: detection boundary minimaxity} if the true sparsity level $\kt$ is unknown \item[Q2.] What is the optimal procedure in absence of accurate sparsity information?  
\end{enumerate}
To facilitate the definition of adaptivity, we consider the case of two sparsity levels, $\kt\leq \ku$. Here $\kt$ denotes the true sparsity level, which is typically not available in practice while $\ku$ denotes the prior knowledge of an upper bound for the sparsity level. If we do not have a good prior knowledge about the sparsity level $s$, then $\ku$ can be much larger than $\kt$. To answer the aforementioned questions on adaptivity, we assume that only the upper bound $\ku$ is known instead of the exact sparsity level $\kt$.
As a consequence, a testing procedure needs to be constructed with the size uniformly controlled over the parameter space $\HH_0(\ku),$
\begin{equation}
%\begin{equation}
{\alphab}(\ku,\phi)=\sup_{\theta\in \HH_0(\ku)} \E_{\theta} \phi \leq \alpha. 
\label{eq: type I error adaptivity}
%\end{equation}
\end{equation}
In contrast to \eqref{eq: type I error}, the control of size is with respect to $\HH_0(\ku)$, a larger parameter space  than $\HH_0(\kt)$, due to the fact that the true sparsity level is unknown. 
%However, when we define the power of the proposed testing procedure, we only evaluate the power over the parameter space with the true sparsity level $\kt$ since that is where the alternative hypothesis belongs to. That is, the power function of a given test $\phi$ is defined as  $\omegab(\kt,\tau,\phi)$ defined in \eqref{eq: power definition}. Using a similar idea to 
Similar to \eqref{eq: detection boundary minimaxity}, we define the adaptive detection boundary $\tauadpt$ as
%\begin{equation}
\begin{equation}
\tauadpt=\arg\min_{\tau}\left\{\tau: \sup_{\phi:\alphab(\ku,\phi)\leq \alpha}\omegab(\kt,\tau,\phi)\geq 1-\eta\right\}.
\label{eq: detection boundary adaptivity}
\end{equation}
%This quantity $\tauadpt$ will be referred to as the adaptive detection boundary of \eqref{eq: testing problem}.
Comparing \eqref{eq: detection boundary adaptivity} with \eqref{eq: detection boundary minimaxity}, the imprecise information about the sparsity level only affects the control of size, where the power functions in \eqref{eq: detection boundary adaptivity} and \eqref{eq: detection boundary minimaxity} are evaluated over the same parameter space, $\HH_1(\kt,\tau)$.
 If a test $\phi$ satisfies the following property,\begin{equation}
\alphab(\ku,\phi)\leq \alpha \quad \text{and} \quad \omegab(\kt,\tau,\phi)\geq 1-\eta \quad \text{for}\;\; \tau \asymp \tauadpt
\label{eq: adaptive optimal}
\end{equation}
then $\phi$ is defined to be adaptive optimal. The question Q2 can be addressed using the adaptive detection boundary $\tauadpt$ and an adaptive optimal test would be the best that we can aim for if there is lack of accurate information on sparsity. 

%For the case $\ku=\kt$, we have $\taumini=\tauadpt$. 
The quantities $\taumini$ and $\tauadpt$ do not depend on the specific testing procedure but mainly reflect the difficulty of the testing problem \eqref{eq: testing problem}, which depends on the parameter space and also the loading vector $\bx_{\rm new}$. The question {Q1} can be addressed through comparing $\taumini$ and $\tauadpt$; if $\taumini \asymp \tauadpt,$ then the hypothesis testing problem \eqref{eq: testing problem} is defined to be adaptive, that is, even if one does not know the exact sparsity level, it is possible to construct a test as if the sparsity level is known; in contrast, if $\taumini \ll \tauadpt,$ the hypothesis testing problem \eqref{eq: testing problem} is defined to be not adaptive. The information on the sparsity level is crucial. In this case, the adaptive detection boundary itself is of great interest as it quantifies the effect of the knowledge of sparsity level. 

As a concluding remark, the minimax detection boundary characterizes the difficulty of the testing problem for the case of known sparsity level while the adaptive detection boundary characterizes a more challenging problem due to the unknown sparsity. The adaptive optimal test satisfying \eqref{eq: adaptive optimal} is more useful in practice than that of a minimax optimal test because the exact sparsity level is typically unknown in applications. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Detection Boundary for Testing Problem \eqref{eq: testing problem}}
\label{sec: results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In this section, we discuss the optimality of the  testing problem \eqref{eq: testing problem} under the optimality framework introduced in Section \ref{sec: framework}. 
We now demonstrate the optimality of the proposed procedure by considering the following two types of loadings $\bx_{\rm new}$, Exact Loading and Decaying Loading.\\
%
%To demonstrate the optimality of the proposed procedure, we focus on the following two types of loadings $\bx_{\rm new}$
%To illustrate the application of the lower bound in Theorem \ref{thm: general lower}, we will address the following two types of 
%\begin{enumerate}
\noindent (E) {\bf Exact Loading.} $\bx_{\rm new}$ is defined as an exact loading if it satisfies,
\begin{equation}
c_0\leq \max_{\{i: \bx_{\rm new, i}\neq 0\}}\left|\bx_{\rm new, i}\right|/\min_{\{i: \bx_{\rm new, i}\neq 0\}}\left|\bx_{\rm new, i}\right|\leq C_0,
\label{eq: exact loading}
\end{equation}
for some positive constants $C_0\geq c_0>0$. The condition \eqref{eq: exact loading} assumes that all non-zero coefficients of the loading vector $\bx_{\rm new}$ are of the same order of magnitude
and hence the complexity of an exact loading $\bx_{\rm new}$ is captured by its sparsity level.  We calibrate the sparsity levels of the regression vectors and the exact loading $\bx_{\rm new}$ as
\begin{equation}
\kt=p^{\gamma},\quad \ku=p^{\gamma_{u}}, \quad \|\bx_{\rm new}\|_0=p^{\gamma_{\rm new}} \; \text{for} \quad 0\leq \gamma< \gamma_{u} \leq 1,\; 0\leq  \gamma_{\rm new} \leq 1.
\label{eq: cal of beta}
\end{equation}
Based on the sparsity level of $\bx_{\rm new}$, we define the following types of loadings,
\begin{enumerate}
\item [(E1)] $\bx_{\rm new}$ is called an {\em exact sparse loading} if it satisfies \eqref{eq: exact loading} with $\gamma_{\rm new}\leq 2 \gamma$; 
\item [(E2)] $\bx_{\rm new}$ is called an {\em exact dense loading} if it satisfies \eqref{eq: exact loading} with $\gamma_{\rm new}>2 \gamma$; 
\end{enumerate} 

Exact loadings are commonly seen in the genetic studies, where the loading $\bx_{\rm new}$ represents a specific observation's SNP and only takes the value from $\{0,1,2\}$.

\medskip
\noindent (D) {\bf Decaying Loading.} Let 
$|x_{\rm new, (1)}|\geq \left|x_{\rm new, (2)}\right|\geq \cdots \geq \left|x_{\rm new, (p)}\right|$ be the sorted coordinates of $\left|\bx_{\rm new}\right|$.
We say that $\bx_{\rm new}$ is decaying at the rate $\delta$ if 
\begin{equation}
\left|x_{\rm new, (i)}\right| \asymp i^{-\delta} \quad \text{for some constant } \delta\geq 0.
\label{eq: decaying}
\end{equation}
Depending on the decaying rate $\delta$, we define the following two types of loadings,
\begin{enumerate}
\item [(D1)] $\bx_{\rm new}$ is called a {\em fast decaying loading} if it satisfies \eqref{eq: decaying} with $\delta\geq \frac{1}{2}$; 
\item [(D2)] $\bx_{\rm new}$ is called a {\em slow decaying loading} if it satisfies \eqref{eq: decaying} with  $0\leq \delta<\frac{1}{2}$.
\end{enumerate}

%\end{enumerate}



%We will apply the general detection boundary result Theorem \ref{thm: general lower} and present the optimality results for testing on the exact sparse loading in Section \ref{sec: exact} and the decaying loading in Section \ref{sec: decaying}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Exact Sparse Loading}
%\label{sec: exact}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%We first focus on the loading $\xi$ with the same order of magnitude, that is, 
%
%
%%and then we control the sparsity of such loadings by $\ell_0$ norm, that is,
%%\begin{equation}
%For a loading $\xi$ satisfying \eqref{eq: equal loading}, its complexity is measured by the sparsity of the loading, which is denoted as . The following theorem shows that the detection boundary $\taumini$ depends on the loading's sparsity level $q$. 
%%\end{equation}
%

To simplify the presentation, we present the optimality results for the case $n_1\asymp n_2$, denoted by $n$ and the results can be extended to the case where $n_1$ and $n_2$ are of different orders. 
We focus on the exact loading and give a summary of the results for the decaying loading in Table \ref{tab: decaying theory}.
The detailed results about decaying loadings will be deferred to Section \ref{sec: decaying} in the supplement. The following theorem establishes the lower bounds for the adaptive detection boundary for exact loadings.
\begin{Theorem}
Suppose that  $s\leq \ku \lesssim {n}/{\log p}$. We calibrate $\kt, \ku$ and $\|\bx_{\rm new}\|_0$ by $\gamma$, $\gamma_{u}$ and $\gamma_{\rm new}$, respectively, as defined in \eqref{eq: cal of beta}.  %We have the following lower bounds for $\tauadpt,$ 
\begin{enumerate}
\item[\rm (E1)] If $\bx_{\rm new}$ is an exact sparse loading, then %with $\gamma_{\rm new}\leq 2 \gamma,$ then 
\begin{equation}
\tauadpt \gtrsim \frac{\sqrt{\|\bx_{\rm new}\|_0}\|\bx_{\rm new}\|_{\infty}}{\sqrt{n}} \asymp \frac{\|\bx_{\rm new}\|_2}{\sqrt{n}}; %\frac{1}{\sqrt{n}} \max\left\{\sqrt{\sum_{j=1}^{s}x_{\rm new,j}^2}, \sqrt{L}\|\bx_{\rm new}\|_{\infty}\right\}
\label{eq: E1}
\end{equation}
%{\red What's $L$?}
%and hence $\taumini\asymp \tauadpt.$
\item[\rm (E2)] If $\bx_{\rm new}$ is an exact dense loading, then %with $\gamma_{\rm new}> 2 \gamma$, then 
\begin{equation}
\tauadpt \gtrsim \begin{cases} \|x_{\rm new}\|_{\infty}\ku \sqrt{\frac{\log p}{n}}&\text{if}\quad \gamma_{\rm new}> 2\gamma_{u};\\
 \frac{\|\bx_{\rm new}\|_2}{\sqrt{n}} & \text{if}\quad \gamma_{\rm new} \le 2\gamma_{u}.
 \end{cases}
 \label{eq: E2}
\end{equation}
%\end{enumerate}
\end{enumerate}
\label{thm: exact sparse lower}
\end{Theorem}

We shall point out here that establishing the adaptive detection boundaries in Theorem \ref{thm: exact sparse lower} requires technical novelty.
A closely related problem, adaptivity of confidence sets, has been carefully studied in the context of high-dimensional linear regression \citep{nickl2013confidence,cai2015regci,cai2018accuracy}. However, it requires new technical tools to establish the adaptive detection boundaries, due to the different geometries demonstrated in Figure \ref{fig: tool different}. 
The main idea of constructing the lower bounds in \citet{nickl2013confidence,cai2015regci,cai2018accuracy} is illustrated in Figure 2(a), where one interior point is first chosen in the smaller parameter space $\Theta(\kt)$ and the corresponding least favorable set is constructed in the larger parameter space $\Theta(\ku)$ such that they are not distinguishable. 
%in the alternative hypothesis space while the hypothesis testing problem is to construct the perturbation in the null hypothesis parameter space.

In comparison to Figure 2(a), the lower bound construction for the testing problem related to Figure 2(b) is more challenging due to the fact that the alternative parameter space $\HH_1(\ku,\tau)$ does not contain the indifference region $0<\bx_{\rm new}^{\intercal}(\bbeta_1-\bbeta_2)<\tau$.  A new technique, {\em transferring technique}, is developed for establishing the sharp lower bounds for the adaptive detection boundary. Define the index of $\bx_{\rm new}$ with the largest absolute value as $i_{\max}=\arg\max|\bx_{\rm new, i}|.$ In constructing the least favorable set in $\HH_0(\ku)$, we first perturb the regression coefficients at other locations except for $i_{\rm max}$ and then choose the regression coefficient at $i_{\rm max}$ such that $\bx_{\rm new,i_{\rm max}}(\bbeta_{1,i_{\rm max}}-\bbeta_{2,i_{\rm max}})>0$ and $\bx_{\rm new}^{\intercal}(\bbeta_1-\bbeta_2)\leq 0$; in construction of the corresponding least favorable set in $\HH_1(\kt,\tau)$, we simply set the regression coefficient with index $i_{\max}$ to be the same as the corresponding coefficient at $i_{\max}$ in $\HH_0(\ku)$  and set all other coefficients to be zero. The above construction is transferring the parameter space complexity from $\HH_0(\ku)$ to $\HH_1(\kt,\tau)$ by matching the regression coefficient at $i_{\max}$. Such a transferring technique can be of independent interest in establishing the adaptive detection boundaries  for other inference problems. 


\begin{figure}[htb]
\scalebox{.6}{
  \begin{subfigure}[b]{0.48\textwidth}
   \begin{tikzpicture}
\draw[black,thick] (2,2) circle (1.5cm);
\draw[black,thick,dashed] (2,2) circle (3cm);
 \draw (2,1.6) node[above]{$\Theta_0(\kt)$};
 \draw (4,3) node[above]{$\Theta_1(\ku)$};
\end{tikzpicture}
    \caption{}
    \label{fig:1}
  \end{subfigure}
  \begin{subfigure}[b]{0.44\textwidth}
  %\foreach \start/\stop in {30/60,45/90,135/180,0/180,45/315}
   \begin{tikzpicture}
   \draw[black,thick] (2,2) arc (270:90:3cm);
   \draw[black,thick,dashed] (3,6.5) arc (90:-90:1.5cm);
   \draw[black,thick] (2,2) -- (2,8); 
   \draw[black,thick,dashed] (3,3.5) -- (3,6.5); 
    \draw (1,4.6) node[above]{$\HH_0(\ku)$};
 \draw (3.8,4.6) node[above]{$\HH_1(\kt,\tau)$};
 \draw[->,thick] (2,2.8) to [out=0,in=-250] (3.6,2.6) node[anchor= north]
        {$\bx_{\rm new}^{\intercal}(\bbeta_1-\bbeta_2)=0$};
   \draw[->,thick] (3,4) to [out=0,in=100] (5,3.5) node[anchor= north]
        {$\bx_{\rm new}^{\intercal}(\bbeta_1-\bbeta_2)=\tau$};      
    \end{tikzpicture}
    \caption{}
    \label{fig:2}
  \end{subfigure}
  }
  \caption{(a) Null and alternative parameter spaces for the confidence set construction; (b) Null and alternative parameter spaces for the hypothesis testing problem.}
\label{fig: tool different}
\end{figure}



%The detection boundaries in Theorem \ref {thm: exact sparse lower} can be attained under regularity conditions. 
The following corollary presents the matched upper bounds for the detection boundaries established in Theorem \ref{thm: exact sparse lower} over certain regimes.
\begin{Corollary}
\label{cor: exact sparse adapt}
Suppose that  $s\leq \ku \lesssim {\sqrt{n}}/{\log p}$. %Then the minimaxity detection boundary and adaptive detection boundary satisfy
\begin{enumerate}
\item[\rm (E1)] If the loading $\bx_{\rm new}$ is an exact sparse loading, then 
\begin{equation}
\tauadpt \asymp \taumini \asymp \frac{\|\bx_{\rm new}\|_2}{\sqrt{n}}
\label{eq: E1 match}
\end{equation}
\item[\rm (E2)]  If the loading $\bx_{\rm new}$ is an exact dense loading, then the results are divided into the following two cases,
\begin{enumerate}
\item[\rm (E2-a)] If $\gamma< \gamma_{u}< \frac{1}{2}\gamma_{\rm new},$ then 
\begin{equation}
\tauadpt \asymp\|x_{\rm new}\|_{\infty}\ku \sqrt{\frac{\log p}{n}} \gg \taumini \asymp\|x_{\rm new}\|_{\infty} \kt \sqrt{\frac{\log p}{n}}.
\label{eq: E2-a match}
\end{equation}
\item[\rm (E2-b)]  If $\gamma< \frac{1}{2}\gamma_{\rm new}\leq \gamma_{u} ,$ then
\begin{equation}
\tauadpt \asymp \frac{\|\bx_{\rm new}\|_2}{\sqrt{n}}\gg \taumini \asymp \|x_{\rm new}\|_{\infty}\kt \sqrt{\frac{\log p}{n}}.
\label{eq: E2-b match}
\end{equation}
%\item[\rm (E2-c)]  If the knowledge of $\kt$ and $\ku$ satisfies $\frac{1}{2}\gamma_{\rm new}\leq\gamma\leq  \gamma_{u} ,$ then
%\begin{equation}
%\tauadpt \asymp \taumini \asymp \frac{\|\bx_{\rm new}\|_2}{\sqrt{n}}.
%\label{eq: E2-c match}
%\end{equation}
\end{enumerate}
\end{enumerate}
\end{Corollary}
%The detection boundary results reveal the fundamental difficulty of the hypothesis testing problems, which depends on two intrinsic features, 1) the loading $\bx_{\rm new}$ and 2) the dimension $p$, the sample size $n$, sparsity $\kt$ and the knowledge of sparsity $\ku$. 
The question Q1 about the possibility of adaptivity of the testing problem \eqref{eq: testing problem} can be addressed by the above corollary, where the testing problem is adaptive for the exact sparse loading case (E1) but not adaptive for the exact dense loading case (E2). The specific cut-off for the ``dense" and ``sparse" cases occurs at $\gamma_{\rm new}=2\gamma$.
%The exact sparse loading case (E1) is significantly different from the  in terms of the detection boundaries.  %For (E1), the hypothesis testing problem \eqref{eq: testing problem} is adaptive while for (E2), the testing problem \eqref{eq: testing problem} is not adaptive, which is more challenging. 
For the case (E2), depending on the value of $\gamma_{u}$, the adaptive detection boundaries can be quite different. The case (E2-a) corresponds to the case that the exact sparsity level is unknown but the upper bound $\ku$ is relatively precise (both $\gamma$ and $\gamma_u$ are below $1/2 \cdot \gamma_{\rm new}$), then we can utilize the proposed procedure $\phi_{\alpha}$ with the sparsity information $\ku$ to construct a testing procedure matching the adaptive detection boundary. See the detailed construction in Section \ref{sec: sparsity procedure} of the supplement. In contrast, the case (E2-b) corresponds to the setting where the prior knowledge of the upper bound $\ku$ is quite rough. For such a case, the proposed testing procedure $\phi_{\alpha}$ defined in \eqref{eq: test} achieves the adaptive detection boundary $\tauadpt$, but not the minimax detection boundary $\taumini$. 

Beyond answering Q1, we can also address the question Q2 with the following corollary, which considers the practical setting that there is limited information on sparsity and presents a unified optimality result for the case of exact loadings. 
\begin{Corollary}
\label{cor: optimality}
Suppose that  $s\leq \ku \lesssim {\sqrt{n}}/{\log p}$ and $\gamma_{u}\geq \gamma_{\rm new}/2$. Then the testing procedure $\phi_{\alpha}$ in \eqref{eq: test} achieves the adaptive detection boundary $\tauadpt \asymp {\|\bx_{\rm new}\|_2}/{\sqrt{n}}$ for any $\bx_{\rm new}$ satisfying \eqref{eq: exact loading}. 
\end{Corollary}
The above Corollary states that, in absence of accurate sparsity information, the proposed procedure $\phi_{\alpha}$ is an adaptive optimal test for all exact loadings $\bx_{\rm new}$. 
%As a concluding remark, we have shown that the proposed procedure $\phi_{\alpha}$ defined in \eqref{eq: test} is optimal in the following two cases, 1) the loading is sparse; 2) the loading is dense and we do not have precise information on the sparsity level. 
%
%\begin{Corollary}
%\label{cor: decaying adapt}
%Suppose that  $s\leq \ku \lesssim \frac{\sqrt{n}}{\log p}$. 
%%We establish the minimaxity detection boundary and adaptive detection boundary for the decaying loading defined in \eqref{eq: decaying}.
%\begin{enumerate}
%\item[\rm (D1)] If the loading $\bx_{\rm new}$ defined in \eqref{eq: decaying} decays at a fast rate with $\delta\geq \frac{1}{2}$, then 
%\begin{equation}
%\tauadpt \asymp \taumini \asymp \frac{\|\bx_{\rm new}\|_2}{\sqrt{n}}
%\label{eq: D1 match}
%\end{equation}
%In particular, for $\delta=\frac{1}{2}$, the detection boundary holds if $\gamma>0$; otherwise the detection boundary holds up to a $\sqrt{\frac{\log p}{\log s}}$ factor.
%\item[\rm (D2)]  If the loading $\bx_{\rm new}$ defined in \eqref{eq: decaying} decays at a slow rate with $0\leq \delta< \frac{1}{2},$, then the minimaxity detection boundary and adaptive detection boundary hold up to a $\sqrt{\log p}$ order
%\begin{enumerate}
%\item[\rm (D2-a)]  If the true sparsity  $\kt$ and the knowledge of $\ku$ satisfies  satisfies $\gamma< \gamma_{u}\leq \frac{1}{2},$ then
%\begin{equation}
%\tauadpt \asymp \frac{\ku^{1-2\delta}}{\sqrt{{{n}}}}\left(\log p\right)^{\frac{1}{2}-\delta} \gg \taumini \asymp \frac{\kt^{1-2\delta}}{\sqrt{{{n}}}}\left(\log p\right)^{\frac{1}{2}-\delta} .
%\label{eq: D2-a match}
%\end{equation}
%\item[\rm (D2-b)] If the true sparsity $\kt$ and the knowledge of $\ku$ satisfies $\gamma< \frac{1}{2}\leq \gamma_{u},$ then 
%\begin{equation}
%\tauadpt \asymp \sqrt{\frac{p^{1-2\delta}}{{n}}} \gg \taumini \asymp \frac{\kt^{1-2\delta}}{\sqrt{{{n}}}}\left(\log p\right)^{\frac{1}{2}-\delta}
%\label{eq: D2-b match}
%\end{equation}
%\item[\rm (D2-c)] If the true sparsity $\kt$ and the knowledge of $\ku$ satisfies $\frac{1}{2}\leq \gamma< \gamma_{u},$ then
%\begin{equation}
%\tauadpt \asymp \taumini  \asymp \sqrt{\frac{p^{1-2\delta}}{{n}}}
%\label{eq: D2-c match}
%\end{equation}
%\end{enumerate}
%\end{enumerate}
%\end{Corollary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparison with Existing Optimality Results on CI}
\label{sec: comparison}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
It is helpful to compare the established optimality results to the related work \citet{cai2015regci} on the minimaxity and adaptivity of confidence intervals for the linear contrast in the one-sample high-dimensional regression. 
%Although the results in the current paper are considering two regression models simultaneously, the optimality results can be directly applied to the one-sample case as the regression coefficient $\bbeta_2$ is set to be zero in the technical analysis. 
Beyond the technical difference highlighted in Figure \ref{fig: tool different}, we also observed the following three distinct features between the present paper and  \citet{cai2015regci}.
\begin{enumerate}
\item[1] The current paper closes the gap between the definitions of exact sparse and dense loading in \citet{cai2015regci}, where the lower bounds for exact sparse loading only covered the case $\gamma_{\rm new}\leq \gamma$ instead of the complete regime $\gamma_{\rm new}\leq 2\gamma$ defined in the current paper. 
\item[2] The result in the current paper considers the additional setting (E2-b) than those in \citet{cai2015regci}, which corresponds to the case where the knowledge on the sparsity level is rough. This additional result is not only of technical interest, but is of broad implications to practical applications. It addresses the important question, ``what is the optimal testing procedure in a practical setting where no accurate sparsity information is available? " As shown in Corollary \ref{cor: optimality}, the proposed procedure $\phi_{\alpha}$ is an adaptive optimal test for all exact loadings $\bx_{\rm new}.$
\item[3] In addition, the technical tools for general loading $\bxnew$ have been developed in Theorem \ref{thm: general lower}, which can handle the loadings not considered in \citet{cai2015regci}. Specifically, we summarize in Table \ref{tab: decaying theory} the optimality results for the decaying loading defined in \eqref{eq: decaying}. As shown in Table \ref{tab: decaying theory}, the fast decaying loading (D1) is similar to the exact sparse loading (E1) while the slow decaying loading (D2) is similar to the exact dense loading (E2). In contrast, the decaying loading has the distinct setting (D2-c) from the exact loading case where the hypothesis testing problem \eqref{eq: testing problem} is adaptive if both $\gamma$ and $\gamma_{u}$ are above $1/2$. See the detailed discussion in Section \ref{sec: decaying} of the supplement.
\end{enumerate}
\begin{table}[htb]
%\centering
%\scalebox{0.75}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
$\delta$&Setting& $\gamma,\gamma_u$&$\taumini$&Rel&$\tauadpt$ &Adpt\\
\hline
$[{1}/{2},\infty)$& (D1)& $\gamma<\gamma_u$& ${\|\bx_{\rm new}\|_2}/{\sqrt{n}}$&$\asymp$&${\|\bx_{\rm new}\|_2}/{\sqrt{n}}$&Yes\\ 
\hline 
\multirow{3}{*}{$[0,{1}/{2})$}&(D2-a)&$\gamma< \gamma_{u}\leq \frac{1}{2}$&${\kt^{1-2\delta}}\left(\log p\right)^{\frac{1}{2}-\delta}/{\sqrt{{{n}}}}$&$\ll$&${\ku^{1-2\delta}}\left(\log p\right)^{\frac{1}{2}-\delta}/{\sqrt{{{n}}}}$&No\\
&(D2-b)&$\gamma< \frac{1}{2}\leq \gamma_{u}$&${\kt^{1-2\delta}}\left(\log p\right)^{\frac{1}{2}-\delta}/{\sqrt{{{n}}}}$&$\ll$&${\|\bx_{\rm new}\|_2}/{\sqrt{n}}$&No\\
&(D2-c)&$\frac{1}{2}\leq \gamma<\gamma_{u}$& ${\|\bx_{\rm new}\|_2}/{\sqrt{n}}$&$\asymp$&${\|\bx_{\rm new}\|_2}/{\sqrt{n}}$&Yes\\
% \hiline
%\multirow{3}{*}{0}  \\
%&200& 0.98 & 0.93 & 0.97 & 0.97 & 3.00 & 3.45 & 0.69 & 0.05 & 0.69 & 0.35 & 0.28 & 0.21 & 0.83 & 0.05 & 0.83 \\ 
%   &  300&1.00 & 1.00 & 0.97 & 0.97 & 2.17 & 2.74 & 0.51 & 0.09 & 0.50 & 0.29 & 0.23 & 0.17 & 0.63 & 0.03 & 0.63 \\ 
%   & 400& 1.00 & 1.00 & 0.95 & 0.94 & 1.94 & 2.33 & 0.50 & 0.05 & 0.50 & 0.25 & 0.20 & 0.15 & 0.61 & 0.00 & 0.61 \\ 
    \hline
\end{tabular}
%}
\caption{Optimality for the decaying loading $\bx_{\rm new}$ defined in \eqref{eq: decaying} over the regime $s\lesssim \ku\lesssim {\sqrt{n}}/{\log p}$. The column indexed with ``Rel" compares $\taumini$ and $\tauadpt$ and the column indexed with ``Adpt" reports whether the testing problem is adaptive or not for the corresponding setting.}
\label{tab: decaying theory}
\end{table}

%%\label{thm: fast decay unknown sparsity}
%%The following theorem characterizes what if the sparsity level is totally unknown.
%%\begin{Theorem}
%%Suppose that $\kt$ denotes the exact sparsity of the detection parameter space and satisfies  $\kt \lesssim\min\left\{\frac{n}{\log p},p^{\gamma}\right\}$ for some constant $0\leq \gamma<\frac{1}{2}$. The detection boundary for the problem ${\left\{ \;\xi^{\intercal}\beta\leq 0\right\}}$ over $\left\{\|\beta\|_0\leq \kt, \xi^{\intercal}\beta\geq  \tau\right\}$.
%%\begin{enumerate}
%%\item For $\delta>\frac{1}{2}$, then we have  $\taumini\asymp \frac{1}{\sqrt{n}}$ such that
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{does not reject} \; H_0\right)\right)\rightarrow 1.
%%\label{eq: total case1}
%%\end{equation}
%%If $\tau\gtrsim {\frac{1}{\sqrt{n}}}$, then then we have  a testing procedure $\phi^{*}$ such that
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{ \left\{\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi^{*} \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi^{*} \; \text{does not reject} \; H_0\right)\right)\rightarrow \alpha.
%%\label{eq: total case1 upper}
%%\end{equation}
%%\item For $\delta=\frac{1}{2}$, then we have  $\taumini\asymp \sqrt{\frac{\log \kt }{{n}}}$,
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{does not reject} \; H_0\right)\right)\rightarrow 1.
%%\label{eq: total case2}
%%\end{equation}
%%If $\tau\gtrsim \sqrt{\frac{\log p }{{n}}}$, then then we have  a testing procedure $\phi^{*}$ such that
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi^{*} \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi^{*} \; \text{does not reject} \; H_0\right)\right)\rightarrow \alpha.
%%\label{eq: total case2 upper}
%%\end{equation}
%
%%\item For $0\leq \delta<\frac{1}{2}$, then we have  $\taumini\asymp \sqrt{\frac{p^{1-2\delta}}{{n}}}$,
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{does not reject} \; H_0\right)\right)\rightarrow 1.
%%\label{eq: total case2}
%%\end{equation}
%%If $\tau\gtrsim \sqrt{\frac{p^{1-2\delta}}{{n}}}$, then then we have  a testing procedure $\phi^{*}$ such that
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi^{*} \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi^{*} \; \text{does not reject} \; H_0\right)\right)\rightarrow \alpha.
%%\label{eq: total case2 upper}
%%\end{equation}
%%\item For $\delta=0$
%%\end{enumerate}
%%\end{Theorem}
%
%Theorem \ref{thm: fast decay two level sparsity} states that for a fast decaying loading with $\delta>1/2$, for $\tau\gtrsim \frac{\|\xi\|_2}{\sqrt{n}}$, we can distinguish $H_1: \xi^{\intercal}\left(\beta-\gamma\right)\geq \tau$ from $H_0: \xi^{\intercal}\left(\beta-\gamma\right)\leq 0$. However, if $\tau\ll \frac{\|\xi\|_2}{\sqrt{n}}$, it is impossible to distinguish the alternative from the null. For the case $\delta=1/2$ and $\kt=c p^{\gamma}$ with $0<\gamma<\frac{1}{2}$, then the upper bound and lower bound for $\tau$ matches and the detection boundary is $\sqrt{\frac{\log p}{n}}$, which is different from the parametric rate $\frac{1}{\sqrt{n}}$ for the case $\delta=\frac{1}{2}$. %we can only distinguish $\left\{\xi^{\intercal}\left(\beta-\gamma\right)\gtrsim \sqrt{\frac{\log p}{{n}}} \right\}$ from $\left\{\xi^{\intercal}\left(\beta-\gamma\right)<0\right\}$. 
%We shall stress that the construction of testing procedure for $\delta=\frac{1}{2}$ does not require any prior knowledge of sparsity $k$ even though $\tau$ is not of the parametric rate.
%
%%\begin{equation}
%%H_0: \xi^{\intercal}\left(\beta-\gamma\right)\leq 0 \quad \text{v.s.} \quad H_1:\xi^{\intercal}\left(\beta-\gamma\right)>0.
%%\label{eq: testing problem}
%%\end{equation}
%%\end{Remark}
%
%%\subsection{Fast decaying loading case $\xi(\delta)$ with $0\leq \delta<\frac{1}{2}$}
%%\subsubsection{Theoretical results}
%
%In the following, we discuss the minimaxity and adaptivity results for the slow-decaying case, which is of fundamental difference from the fast-decaying case.
%\begin{Theorem}
%\label{thm: slow decay two level sparsity}
%Suppose that the two sparsity levels $\kt,\ku$ satisfy  $\kt\leq \ku\lesssim\min\left\{\frac{n}{\log p},p^{\gamma}\right\}$ for some constant $0\leq \gamma<\frac{1}{2}$. %The detection boundary for the problem ${\left\{\|\beta\|_0\leq \ku\;, \;\xi^{\intercal}\left(\beta-\gamma\right)\leq 0\right\}}$ over $\left\{\|\beta\|_0\leq \kt, \xi^{\intercal}\left(\beta-\gamma\right)\geq  \tau\right\}$. %$H_0: \xi^{\intercal}\left(\beta-\gamma\right)\leq 0, \beta\in \Theta(\ku)$ over $H_1: \xi^{\intercal}\left(\beta-\gamma\right)>0,\beta\in \Theta(\kt)$,
%\begin{enumerate}
%%\item For $\delta>\frac{1}{2}$, then we have  $\taumini\asymp \frac{1}{\sqrt{n}}$ such that
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\left(\beta-\gamma\right)\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\left(\beta-\gamma\right)\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{does not reject} \; H_0\right)\right)\rightarrow 1.
%%\label{eq: k12 case1}
%%\end{equation}
%%If $\tau\gtrsim {\frac{1}{\sqrt{n}}}$, then then we have  a testing procedure $\phi^{*}$ such that
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\left(\beta-\gamma\right)\leq 0\right\}}\PP_{\beta}\left(\phi^{*} \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi^{*} \; \text{does not reject} \; H_0\right)\right)\rightarrow \alpha.
%%\label{eq: k12 case1 upper}
%%\end{equation}
%%\item For $\delta=\frac{1}{2}$, then we have  $\taumini\asymp \sqrt{\frac{\log \kt }{{n}}}$,
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{does not reject} \; H_0\right)\right)\rightarrow 1.
%%\label{eq: k12 case2}
%%\end{equation}
%%If $\tau\gtrsim \sqrt{\frac{\log p }{{n}}}$, then then we have  a testing procedure $\phi^{*}$ such that
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi^{*} \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi^{*} \; \text{does not reject} \; H_0\right)\right)\rightarrow \alpha.
%%\label{eq: k12 case2 upper}
%%\end{equation}
%\item For $0<\delta<\frac{1}{2}$, then we have  $\taumini\asymp \frac{\ku^{1-2\delta}}{\sqrt{{{n}}}}\left(\log p\right)^{\frac{1}{2}-\delta}\sqrt{\frac{\log\left(1+\log(p)\right)}{{\log p}}}$.
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{does not reject} \; H_0\right)\right)\rightarrow 1.
%%\inf_{\phi:\alphab(\ku,\delta,\phi)\leq \alpha}\omegab(\kt,\ku,\delta,\tau)\rightarrow 1-\eta.
%%\label{eq: k12 case3}
%%\end{equation}
%If $\tau\gtrsim \frac{\ku^{1-2\delta}}{\sqrt{{{n}}}}\left(\log p\right)^{\frac{1}{2}-\delta}$, the testing procedure $\phi^{*}_{C}(\ku)$ defined in \eqref{eq: comb nonlinear test} satisfies \eqref{eq: minimax test}.
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi^{*} \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi^{*} \; \text{does not reject} \; H_0\right)\right)\rightarrow \alpha.
%%\label{eq: k12 case3 upper}
%%\end{equation}
%\item For $\delta=0$, then we have  $\taumini\asymp \ku\sqrt{\frac{\log p}{{n}}}$.
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{does not reject} \; H_0\right)\right)\rightarrow 1.
%%\inf_{\phi:\alphab(\ku,\delta,\phi)\leq \alpha}\omegab(\kt,\ku,\delta,\tau)\rightarrow 1-\eta.
%%\label{eq: k12 case4}
%%\end{equation}
%If $\tau\gtrsim  \ku\sqrt{\frac{\log p}{{n}}}$, the testing procedure $\phi^{*}_{C}(\ku)$ defined in \eqref{eq: comb nonlinear test} satisfies \eqref{eq: minimax test}.
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi^{*} \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi^{*} \; \text{does not reject} \; H_0\right)\right)\rightarrow \alpha.
%%\label{eq: k12 case4 upper}
%%\end{equation}
%\end{enumerate}
%\end{Theorem}
%
%Theorem \ref{thm: slow decay two level sparsity} states that for a slow decaying loading with $\delta\leq 1/2$, if our prior knowledge of the sparsity level is $\|\beta\|_0\leq \ku$, then the detection boundary $\tau$ is at least $\taumini\asymp \frac{\ku^{1-2\delta}}{\sqrt{{{n}}}}\left(\log p\right)^{\frac{1}{2}-\delta}\sqrt{\frac{\log\left(1+\log(p)\right)}{{\log p}}}$. There exists a test which nearly achieves this detection boundary. We shall stress that the detection boundary $\tau$ depends on the prior knowledge of the sparsity $\ku$ of $\beta$. That is, it is impossible to construct an adaptive testing procedure for the slow-decaying loading case, which is fundamentally different from the fast-decaying loading case.  This is of great practical implication since it informs the practitioners of that, for the slow-decaying loading case, the testing problem becomes harder and the detection boundary $\tau$ must be inflated if the accurate sparsity information of $\beta$ is unavailable.
%
%%For the case $\delta=1/2$,we can only distinguish $\left\{\xi^{\intercal}\left(\beta-\gamma\right)\gtrsim \sqrt{\frac{\log p}{{n}}} \right\}$ from $\left\{\xi^{\intercal}\left(\beta-\gamma\right)<0\right\}$. Note that this does not require any prior knowledge of sparsity $k$.
%%\end{Remark}
%
%%The following theorem characterizes what if the sparsity level is totally unknown.
%
%After establishing Theorem \ref{thm: slow decay two level sparsity}, a reminding important question is what is the detection boundary for the slow-decaying loading case if no sparsity information is available. The following theorem will answer this question. 
%\begin{Theorem}
%\label{thm: slow decay unknown sparsity}
%Suppose that $\kt \lesssim \frac{n}{\log p}$, $\kt \leq \ku$ and $\ku\gtrsim \sqrt{p}$. %The detection boundary for the problem ${\left\{ \;\xi^{\intercal}\beta\leq 0\right\}}$ over $\left\{\|\beta\|_0\leq \kt, \xi^{\intercal}\beta\geq  \tau\right\}$.
%%\begin{enumerate}
%%\item For $\delta>\frac{1}{2}$, then we have  $\taumini\asymp \frac{1}{\sqrt{n}}$ such that
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{does not reject} \; H_0\right)\right)\rightarrow 1.
%%\label{eq: total case1}
%%\end{equation}
%%If $\tau\gtrsim {\frac{1}{\sqrt{n}}}$, then then we have  a testing procedure $\phi^{*}$ such that
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{ \left\{\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi^{*} \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi^{*} \; \text{does not reject} \; H_0\right)\right)\rightarrow \alpha.
%%\label{eq: total case1 upper}
%%\end{equation}
%%\item For $\delta=\frac{1}{2}$, then we have  $\taumini\asymp \sqrt{\frac{\log \kt }{{n}}}$,
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{does not reject} \; H_0\right)\right)\rightarrow 1.
%%\label{eq: total case2}
%%\end{equation}
%%If $\tau\gtrsim \sqrt{\frac{\log p }{{n}}}$, then then we have  a testing procedure $\phi^{*}$ such that
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi^{*} \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi^{*} \; \text{does not reject} \; H_0\right)\right)\rightarrow \alpha.
%%\label{eq: total case2 upper}
%%\end{equation}
%%
%For $0\leq \delta<\frac{1}{2}$, then we have  $\taumini\asymp \sqrt{\frac{p^{1-2\delta}}{{n}}}$.
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{does not reject} \; H_0\right)\right)\rightarrow 1.
%%\inf_{\phi:\alphab(p,\delta,\phi)\leq \alpha}\omegab(\kt,p,\delta,\tau)\rightarrow 1-\eta.
%%\label{eq: total case2}
%%\end{equation}
%If $\tau\gtrsim \sqrt{\frac{p^{1-2\delta}}{{n}}}$, the testing procedure $\phi_{\alpha}$ defined in \eqref{eq: test} satisfies \eqref{eq: minimax test}.
%%satisfies the following property,
%%\begin{equation}
%%\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi^{*} \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi^{*} \; \text{does not reject} \; H_0\right)\right)\rightarrow \alpha.
%%\label{eq: total case2 upper}
%%\end{equation}
%%\item For $\delta=0$
%%\end{enumerate}
%\end{Theorem}
%
%Theorem \ref{thm: slow decay unknown sparsity} states that for a slow decaying loading with $\delta\leq 1/2$, if we do not have any prior knowledge of the sparsity (i.e. $\ku=p\geq \sqrt{p}$), the detection boundary is increased to $\sqrt{\frac{p^{1-2\delta}}{{n}}}$ and such a detection boundary can be achieved by the testing procedure $\phi^{*}_{L}$ introduced in \eqref{eq: linear test}. %We shall stress that the prior knowledge of the sparsity $\ku$ of $\beta$ determines the distinguishable region. %For the case $\delta=1/2$,we can only \
%
%From the empirical point of view, we first need to classify the decaying rate $\delta$ of the observation $\xi(\delta)$. Then based on the decaying rate, we have the following recommendations,
%\begin{enumerate}
%\item For the case $\delta\geq 1/2$, we recommend the testing procedure $\phi_{\alpha}$ defined in \eqref{eq: test}.
%\item For the case $0\leq \delta <1/2$, if the prior information of the sparsity level $\ku$ is available and $\ku \lesssim \sqrt{p}$, we recommend the testing procedure $\phi^{*}_{C}(k)$ introduced in \eqref{eq: comb nonlinear test}. Otherwise, we recommend the testing procedure $\phi_{\alpha}$ defined in \eqref{eq: test}.%={\mathbf 1}\left(\widehat{\mu}(k)-\rho(\xi,k)>0\right).
%%\label
%%\item For the case $0\leq \delta <1/2$, if we do not have prior knowledge of sparsity level
%\end{enumerate}


%
%\underline{Special case on $\delta=0$}\\
%We first consider the loading
%\begin{equation}
%\xi=\left(1,1,\cdots,1\right).
%\label{eq: dense loading}
%\end{equation}
%For this case, we consider the following least favorable spaces with $\rho>0$,
%\begin{equation}
%\begin{aligned}
%\FF_1&=\left\{\left(\left({\ku-1}\right)\rho, \beta_{-1}\right): \beta_{-1}\in \mathcal{R}^{p-1}, \|\beta_{-1}\|_0=\ku-1, \beta_{j} \in \left\{0,-\rho\right\} \; \text{for} \; 2\leq j\leq p\right\}\\
%\FF_2&=\left\{\left(\left({\ku-1}\right)\rho,\mathbf{0}_{p-1}\right)\right\}
%\end{aligned}
%\end{equation}
%Let $\tau=\left({\ku-1}\right)\rho$. Since $\xi^{\intercal}\beta=0$ for $\beta\in \FF_1$, we have
%\begin{equation}
%\FF_1 \subset \left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\beta\leq 0\right\} \quad \text{and} \quad \FF_2\subset \left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}
%\end{equation}
%Let $\pi_1$ denote the uniform prior over the parameter space $\FF_1$ and $\pi_2$ denote the point mass on $\FF_2$. Then we have, if $\rho=c\sqrt{\frac{\log p}{n}}$, then we have
%\begin{equation}
%{\rm TV}\left(f_{\pi_1},f_{\pi_2}\right)\rightarrow 0.
%\end{equation}
%Hence
%\begin{equation}
%\inf_{0\leq \phi \leq 1}\left(\PP_{\pi_1}\left(\phi \; \text{rejects} \; H_0\right)+\PP_{\pi_2}\left(\phi \; \text{does not reject} \; H_0\right)\right)=1-{\rm TV}\left(f_{\pi_1},f_{\pi_2}\right)\rightarrow 1.
%\end{equation}
%Note that for any test $0\leq \phi \leq 1$, if $\taumini\asymp \ku\sqrt{\frac{\log p}{n}}$, then
%\begin{equation}
%\begin{aligned}
%%&\inf_{}\left(\right)\\
%&\text{size}\; +\; \text{Type II error}\\
%=&\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{does not reject} \; H_0\right)\right)\\
%=&\sup_{\left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+1-\inf_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)\\
%\geq &\PP_{\pi_1}\left(\phi \; \text{rejects} \; H_0\right)+\PP_{\pi_2}\left(\phi \; \text{does not reject} \; H_0\right)\rightarrow 1.
%\end{aligned}
%\end{equation}
%By the above equation, we have shown that the detection boundary is
%\begin{equation}
%\Theta(\kt, C \ku\sqrt{\frac{\log p}{n}})=\left\{\|\beta\|_0\leq \kt, \xi^{\intercal}\beta\geq  C \ku\sqrt{\frac{\log p}{n}}\right\}.
%\label{eq: detection boundary delta=0}
%\end{equation}
%\underline{Special case on $0<\delta<\frac{1}{2}$}
%We first consider the loading
%\begin{equation}
%\xi=\left(1^{-\delta},2^{-\delta},\cdots,j^{-\delta},\cdots,p^{-\delta}\right).
%\label{eq: dense decay loading}
%\end{equation}
%For this case, we consider the following least favorable spaces with $\rho>0$,
%\begin{equation}
%\begin{aligned}
%\FF_1&=\left\{\left(S(\ku,l)\rho, \nu,\mathbf{0}_{p-l}\right): \nu\in \mathcal{R}^{l}, \|\nu\|_0=\ku-1, \beta_{j} \in \left\{0,-\rho\right\} \; \text{for} \; 2\leq j\leq l+1\right\}\\
%\FF_2&=\left\{\left(S(\ku,l)\rho,\mathbf{0}_{p-1}\right)\right\},
%\end{aligned}
%\end{equation}
%where
%\begin{equation}
%S(\ku,l)=\sum_{j=l+3-\ku}^{l+1} j^{-\delta}.
%\end{equation}
%Let $\tau=S(\ku,l)\rho$. Since $\xi^{\intercal}\beta\leq 0$ for $\beta \in \FF_1$ we have
%\begin{equation}
%\FF_1 \subset \left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\beta\leq 0\right\} \quad \text{and} \quad \FF_2\subset \left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}
%\end{equation}
%Let $\pi_1$ denote the uniform prior over the parameter space $\FF_1$ and $\pi_2$ denote the point mass on $\FF_2$. Then we have, if $\rho=c\sqrt{\frac{\log p}{n}}$, then we have
%\begin{equation}
%{\rm TV}\left(f_{\pi_1},f_{\pi_2}\right)\rightarrow 0.
%\end{equation}
%Hence
%\begin{equation}
%\inf_{0\leq \phi \leq 1}\left(\PP_{\pi_1}\left(\phi \; \text{rejects} \; H_0\right)+\PP_{\pi_2}\left(\phi \; \text{does not reject} \; H_0\right)\right)=1-{\rm TV}\left(f_{\pi_1},f_{\pi_2}\right)\rightarrow 1.
%\end{equation}
%Note that for any test $0\leq \phi \leq 1$, if $\taumini\asymp S(\ku,l)\rho$, then
%\begin{equation}
%\begin{aligned}
%%&\inf_{}\left(\right)\\
%&\text{size}\; +\; \text{Type II error}\\
%=&\sup_{\xi \in \Gamma_{W}\left(\delta\right)}\left(\sup_{\left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+\sup_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{does not reject} \; H_0\right)\right)\\
%=&\sup_{\left\{\|\beta\|_0\leq \ku\; , \;\xi^{\intercal}\beta\leq 0\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)+1-\inf_{\left\{\|\beta\|_0\leq \kt\; , \; \xi^{\intercal}\beta\geq \tau\right\}}\PP_{\beta}\left(\phi \; \text{rejects} \; H_0\right)\\
%\geq &\PP_{\pi_1}\left(\phi \; \text{rejects} \; H_0\right)+\PP_{\pi_2}\left(\phi \; \text{does not reject} \; H_0\right)\rightarrow 1.
%\end{aligned}
%\end{equation}
%By the above equation, we have shown that the detection boundary is
%\begin{equation}
%\Theta(\kt, S(\ku,l)\rho)=\left\{\|\beta\|_0\leq \kt, \xi^{\intercal}\beta\geq  S(\ku,l)\rho\right\}.
%%\label{eq: detection boundary}
%\end{equation}
%
%

%\newpage
%
%
%{\blue \bf The following results might not be included in the finalized paper. }
%\section{Decay Loading}
%
%
%\subsection{Hypothesis testing with decay loadings}
%
%In last section, we focus on the case that the loading is exactly sparse. In this section, we will discuss the case where the loading is approximately sparse,
%\begin{equation}
%|\xi|_{(1)}\geq |\xi|_{(2)}\geq |\xi|_{(3)} \cdots \geq |\xi|_{(p)} \quad \text{and} \quad |\xi|_{(j)}\asymp j^{-\delta}.
%\label{eq: decay loading}
%\end{equation}
%
%
%\begin{center}
%\begin{tabular}{ |c|c|c|c|}
% \hline
%Loading Name & $\xi$ \\
%\hline
%Sparse Loading&$\xi$ satisfying \eqref{eq: exact loading} with $\|\xi_0\|\lesssim k^{2}$\\
%\hline
%Dense Loading&$\xi$ satisfying \eqref{eq: exact loading} with $\|\xi_0\|\gg k^{2}$\\
%\hline
%Fast-Decay Loading&$\xi$ satisfying \eqref{eq: decay loading} with $\delta\geq \frac{1}{2}$\\
%\hline
%Slow-Decay Loading&$\xi$ satisfying \eqref{eq: decay loading} with $0\leq \delta<\frac{1}{2}$\\
%\hline
%\end{tabular}
%\end{center}
%
%
%%\subsection{Testing procedure}
%In this section, we introduce another procedure using additional sparsity information. In contrast to the procedure proposed in \eqref{sec: sparsity procedure1}, the following construction applies the idea developed in section \ref{sec: no sparisty} to those coordinates corresponding to large $\left|\bx_{\rm new, i}\right|$ and applies the idea developed in section \ref{sec: sparsity procedure1} to other coordinates corresponding to small $\left|\bx_{\rm new, i}\right|$.
%
%Without loss of generality, we can assume the loading $\xi$ with the following ordering,
%\begin{equation}
%\left|\xi_1\right|\geq \left|\xi_2\right|\geq \left|\xi_3\right|\geq \cdots \geq \left|\xi_p\right|.
%\label{eq: aligned xi}
%\end{equation}
%%We define $\omega=\beta-\gamma$
%
%We define $\widehat{\beta-\gamma}$ to be the following hard-thresholding estimator, for $1\leq j\leq p,$
%\begin{equation}
%\widehat{\beta-\gamma}_j=\left(\widetilde{\beta}_j-\widetilde{\gamma}_j\right) \times {\mathbf 1}\left\{\left|\frac{\widetilde{\beta}_j-\widetilde{\gamma}_j}{\sqrt{e_j^{\intercal}\left(\sigma_1^2\Sigma^{-1}\widehat{\Sigma}\Sigma^{-1}+\sigma_2^2 \Gamma^{-1}\widehat{\Gamma}\Gamma^{-1}\right)e_j}}  \right|\geq \sqrt{\frac{2.01\log p}{{n_2}}} \right\}.
%\label{eq: hard threshold debiased}
%\end{equation}
%Note that $\sqrt{e_j^{\intercal}\left(\sigma_1^2\Sigma^{-1}\widehat{\Sigma}\Sigma^{-1}+\sigma_2^2 \Gamma^{-1}\widehat{\Gamma}\Gamma^{-1}\right)e_j}$ is the standard error of $\left(\widetilde{\beta}_j-\widetilde{\gamma}_j\right)$. For small $|\widetilde{\beta}_j-\widetilde{\gamma}_j|$, $\widehat{\beta-\gamma}_j$ is set as zero while for large $|\widetilde{\beta}_j-\widetilde{\gamma}_j|$, $\widehat{\beta-\gamma}_j$ is set as $\widetilde{\beta}_j-\widetilde{\gamma}_j$.
%We propose the following estimator of $\mu=\xi^{\intercal}\left(\beta-\gamma\right)$
%\begin{equation}
%\widehat{\mu}(k)=\sum_{j=1}^{\lfloor k^2\log p \rfloor}  {\xi}_{j} \left(\widetilde{\beta}_j-\widetilde{\gamma}_j\right) +\sum_{j\geq \lfloor k^2\log p \rfloor+1} {\xi}_{j} \widehat{\beta-\gamma}_j .
%\label{eq: combined estimator}
%\end{equation}
%%The estimator $\widehat{\mu}(k)$ consists of two parts, where  
%For large absolute values of $\xi_j$ (corresponding to $1\leq j \leq\lfloor k^2\log p \rfloor$), we plug in the de-biased estimator $\widetilde{\beta}_j-\widetilde{\gamma}_j$; for small absolute values of $\xi_j$ (corresponding to $j \geq \lfloor k^2\log p \rfloor+1$), we plug in the thresholded estimator \eqref{eq: hard threshold debiased}. The intuition of plugging in de-biased estimator for $1\leq j \leq\lfloor k^2\log p \rfloor$ is to remove the bias of scaled Lasso estimator and construct an approximately unbiased estimator. However, for $j \geq \lfloor k^2\log p \rfloor+1$, we plug in the thresholded estimator to avoid an inflation of variance. In short, the fundamental reasoning of $\widehat{\mu}(k)$ in \eqref{eq: combined estimator} is to balance the bias and variance.
%
%
%To quantify the uncertainty of the estimator  $\widehat{\mu}(k)$, we introduce two re-scaled loading vectors $\widehat{\xi}$ and $\bar{\xi}$, defined as,  
%\begin{equation}
%\widetilde{\xi}_j=0 \;\text{for} \;1\leq j\leq \lfloor k^2\log p \rfloor, \quad \widetilde{\xi}_j=\xi_j\sqrt{e_j^{\intercal}\left(\sigma_1^2\Sigma^{-1}\widehat{\Sigma}\Sigma^{-1}+\sigma_2^2 \Gamma^{-1}\widehat{\Gamma}\Gamma^{-1}\right)e_j} \; \text{for} \; \lfloor k^2\log p \rfloor< j\leq p.
%\end{equation}
%\begin{equation}
%\bar{\xi}_j=\xi_j\;\text{for} \;1\leq j\leq \lfloor k^2\log p \rfloor, \quad \bar{\xi}_j=0 \; \text{for} \; \lfloor k^2\log p \rfloor< j\leq p.
%\end{equation}
%Then we can induce the following decision rule,
%\begin{equation}
%\phi^{*}_{C}(k)={\mathbf 1}\left(\widehat{\mu}(k)-\rho(\xi,k)>0\right),
%\label{eq: comb nonlinear test}
%\end{equation}
%where
%$$\rho(\xi,k)=\sqrt{\frac{\bar{\xi}^{\intercal}\left(\sigma_1^2\Sigma^{-1}\widehat{\Sigma}\Sigma^{-1}+\sigma_2^2 \Gamma^{-1}\widehat{\Gamma}\Gamma^{-1}\right)\bar{\xi}}{{n_2}}}+ \sum_{j=1}^{k}\left|\widetilde{\xi}_{(j)}\right| \sqrt{\frac{2.01 \log p}{n_2}},$$
%with $\widetilde{\xi}_{(j)}$ denoting the $j$-th largest absolute value of $\widetilde{\xi}$. Note that $\rho(\xi,k)$ is measuring the uncertainty of the proposed estimator $\widehat{\mu}(k)$, where $\sqrt{\frac{\bar{\xi}^{\intercal}\left(\sigma_1^2\Sigma^{-1}\widehat{\Sigma}\Sigma^{-1}+\sigma_2^2 \Gamma^{-1}\widehat{\Gamma}\Gamma^{-1}\right)\bar{\xi}}{{n_2}}}$ measures the standard error of $\sum_{j=1}^{\lfloor k^2\log p \rfloor}  {\xi}_{j} \left(\widetilde{\beta}_j-\widetilde{\gamma}_j\right)$ and $\sum_{j=1}^{k}\left|\widetilde{\xi}_{(j)}\right| \sqrt{\frac{2.01 \log p}{n_2}}$ is a high probability upper bound for the estimator error $\sum_{j\geq \lfloor k^2\log p \rfloor+1} {\xi}_{j} \left(\widehat{\beta-\gamma}_j-(\beta_j-\gamma_j)\right)$.
%The following theorem shows that the testing procedure constructed in \eqref{eq: comb nonlinear test} has a proper type I error.
%\begin{Proposition} 
%\label{prop: combined test prop}
%Suppose that $k\leq c \frac{n}{\log p}$ for some $c>0$, then we have
%\begin{equation}
%\limsup_{n,p\rightarrow \infty} \sup_{\theta\in \FF_0(s)} \E_{\theta} \phi^{*}_{C}(k) \leq \alpha.
%%\alphab(k,\xi,\phi^{*}_{L})\leq \alpha \quad \text{and} \quad \alphab(k,\xi,\phi^{*}_{T}(k))\leq \alpha.
%\label{eq: combined test}
%\end{equation}
%\end{Proposition}
%

%\end{Remark}
%}



%\section{Construction of Confidence Interval}
%\subsection{Framework for Adaptive Confidence Interval}
%For $0<\alpha<1$ and a given parameter space $\Theta$ and the linear functional $\xi^{\intercal}\beta$, denote by  $\SCIZ$ the set of all $(1-\eta)$ level confidence intervals for $\xi^{\intercal}\left(\beta-\gamma\right)$ over the parameter space $\Theta$,
%\begin{equation}
%\SCIZ=\left\{\CIZg=[l(Z), u(Z)]: \inf_{\theta\in \Theta} \PP(l(Z) \leq \xi^{\intercal}\left(\beta-\gamma\right)\leq u(Z))\rightarrow 1-\eta \right\}.
%\end{equation}
%For any confidence interval $\CIZg \in \SCIZ$, the maximum expected length over a parameter space $\Theta$ is defined as
%$$L({\CIZg},\Theta,\xi)=\sup_{\theta \in \Theta} \E_{\theta} L\left(\CIZg\right),$$
%where for confidence interval $\CIZg=[l(Z), u(Z)]$, $L(\CIZg)= u(Z)-l(Z)$ denotes its length. For two parameter spaces $\Theta_1 \subseteq \Theta$, we define the benchmark $L_{\alpha}^{*}(\Theta_1,\Theta, \xi)$ as the infimum of the maximum expected length over $\Theta_1$ among all $(1-\eta)$-level confidence intervals over $\Theta$,
%\begin{equation}
%L_{\alpha}^{*}(\Theta_1,\Theta,\xi)=\inf_{\CIZg\in \SCIZ} L(\CIZg, \Theta_1,\xi).
%\label{eq: benchmark}
%\end{equation}
%We will write $L_{\alpha}^{*}(\Theta,\xi)$ for $L_{\alpha}^{*}(\Theta,\Theta,\xi)$, which is the minimax expected length of confidence intervals over $\Theta$.
%
%We should emphasize that $L_{\alpha}^{*}(\Theta_1,\Theta,\xi)$ is an important quantity that measures the degree of adaptivity over the nested spaces $\Theta_1\subset \Theta$. A confidence interval $\CIZg$ that is (rate-optimally)  adaptive over $\Theta_1$ and $\Theta$ should have the optimal expected length performance simultaneously over both $\Theta_1$ and $\Theta$ while maintaining a given coverage probability over $\Theta$, i.e.,  $\CIZg\in \SCIZ$ such that
%$$L({\CIZg},\Theta_1,\xi) \asymp L_{\alpha}^{*}(\Theta_1,\xi) \quad  \text{and} \quad L({\CIZg},\Theta,\xi) \asymp L_{\alpha}^{*}(\Theta,\xi).$$ Note that in this case $L({\CIZg},\Theta_1,\xi)\ge L_{\alpha}^{*}(\Theta_1,\Theta,\xi)$. So for  two parameter spaces $\Theta_1\subset \Theta$, if $L_{\alpha}^{*}(\Theta_1,\Theta,\xi) \gg  L_{\alpha}^{*}(\Theta_1,\xi),
%$
%then rate-optimal adaptation between $\Theta_1$ and $\Theta$ is impossible to achieve.
%
%\subsection{Construction of Confidence Interval}
%\begin{enumerate}
%\item Based on the expression \eqref{eq: expression of debiased estimator}, we construct the following confidence interval
%\begin{equation}
%{\rm CI}_{L}=\xi^{\intercal} \left(\widetilde{\beta}-\widetilde{\gamma}\right)+\frac{z_{\alpha/2}}{\sqrt{n_2}}\left(-\xi^{\intercal}\left(\sigma_1^2\Sigma^{-1}\widehat{\Sigma}\Sigma^{-1}+\sigma_2^2 \Gamma^{-1}\widehat{\Gamma}\Gamma^{-1}\right)\xi,+\xi^{\intercal}\left(\sigma_1^2\Sigma^{-1}\widehat{\Sigma}\Sigma^{-1}+\sigma_2^2 \Gamma^{-1}\widehat{\Gamma}\Gamma^{-1}\right)\xi\right)
%\label{eq: linear CI}
%\end{equation}
%\item Based on \eqref{eq: second center of CI}, we construct the confidence interval as
%\begin{equation}
%%\begin{aligned}
%{\rm CI}_{T}(k)=\left(\widehat{\mu}(k)-d(k) \sqrt{\frac{2.01 \log p}{n_2}},\widehat{\mu}+d(k) \sqrt{\frac{2.01 \log p}{n_2}}\right).
%%\end{aligned}
%\label{eq: thresholded CI}
%\end{equation}
%\item Based on \eqref{eq: third center of CI}, we construct the confidence interval as
%\label{eq: third center of CI}
%\begin{equation}
%%\begin{aligned}
%{\rm CI}_{C}(k)=\left(\widehat{\mu}(k)-\rho(\xi,k),\widehat{\mu}+\rho(\xi,k)\right)
%%\end{aligned}
%\label{eq: comb thresholded CI}
%\end{equation}
%where
%$$\rho(\xi,k)=\sqrt{\frac{\bar{\xi}^{\intercal}\left(\sigma_1^2\Sigma^{-1}\widehat{\Sigma}\Sigma^{-1}+\sigma_2^2 \Gamma^{-1}\widehat{\Gamma}\Gamma^{-1}\right)\bar{\xi}}{{n_2}}}+ d(k) \sqrt{\frac{2.01 \log p}{n_2}},$$
%with $\bar{\xi}$ defined as $\bar{\xi}_j=\xi_j$ for $1\leq j \leq \lfloor k^2\log p \rfloor$ and $\bar{\xi}_j=0$ otherwise.
%\end{enumerate}
%
%%\subsection{Decay Loading}
%%For the exact sparsity case, we have the following results for the confidence intervals for $\xi^{\intercal}(\beta-\gamma)$.
%The following theorem establishes the convergence rate for the minimax quantity ${\mathbf L}_{\alpha}^{*}\left(\Theta(\kt), \xi\right)$ and the adaptivity benchmark ${\mathbf L}_{\alpha}^{*}\left(\Theta(\kt), \Theta(\ku),\xi\right)$.
%\begin{Theorem}
%\label{thm: length of CI}
%Suppose that $\kt\leq \ku\leq \frac{n}{\log p}$, $\kt=p^{\gamma_1}$ and$\ku=p^{\gamma_2}$ for $\gamma_1< \frac{1}{2}$ and $\gamma_2< \frac{1}{2}$. Then we have
%\begin{equation}
%{\mathbf L}_{\alpha}^{*}\left(\Theta(\kt), \xi\right) \asymp
%        \begin{cases}
%        \|\xi\|_2/\sqrt{n}& \text{if} \quad \|\xi\|_0\lesssim \kt^2;\\[3pt]
%        %\|\xi\|_{\infty}\sqrt{\|\xi\|_0/n}\asymp\|\xi\|_2/\sqrt{n}& \text{if}\quad \kt\lesssim \|\xi\|_0\lesssim \kt^2;\\[3pt]
%        \|\xi\|_{\infty}\kt\sqrt{2\log p/n} & \text{if}\quad \|\xi\|_0=p^{\gamma_{\rm new}},
%        \end{cases}
%\label{eq: minimax complete}
%\end{equation}
%for some positive constant $2\gamma_1<\gamma_{\rm new}\leq 1$. Also, we have
%\begin{equation}
%{\mathbf L}_{\alpha}^{*}\left(\Theta(\kt), \Theta(\ku),\xi\right) \asymp
%        \begin{cases}
%        \|\xi\|_2/\sqrt{n}& \text{if} \quad \|\xi\|_0\lesssim \ku^2;\\[3pt]
%        %\|\xi\|_{\infty}\sqrt{\|\xi\|_0/n}\asymp\|\xi\|_2/\sqrt{n}& \text{if}\quad \ku\lesssim \|\xi\|_0\lesssim \ku^2;\\[3pt]
%        \|\xi\|_{\infty}\ku\sqrt{2\log p/n} & \text{if}\quad \|\xi\|_0=p^{\gamma_{\rm new}},
%        \end{cases}
%\label{eq: adaptivity complete}
%\end{equation}
%for some positive constant $2\gamma_2<\gamma_{\rm new}\leq 1$.
%\end{Theorem}
%
%The optimal rate $\|\xi\|_2/\sqrt{n}$ in \eqref{eq: minimax complete} and \eqref{eq: adaptivity complete} can be achieved by the confidence interval ${\rm CI}_{L}$ defined in \eqref{eq: linear CI}. The optimal rate $\|\xi\|_{\infty}\kt\sqrt{2\log p/n}$ in \eqref{eq: minimax complete} and $\|\xi\|_{\infty}\kt\sqrt{2\log p/n}$ in \eqref{eq: adaptivity complete} can be achieved by the confidence intervals ${\rm CI}_{T}(\kt)$ and ${\rm CI}_{T}(\ku)$ defined in \eqref{eq: thresholded CI} , respectively.
%
%\begin{Remark}
%By the above theorem, we see that as long as $\|\xi\|_0\lesssim \kt^2$, then we have
%\begin{equation}
%{\mathbf L}_{\alpha}^{*}\left(\Theta(\kt), \xi\right)\asymp {\mathbf L}_{\alpha}^{*}\left(\Theta(\kt), \Theta(\ku),\xi\right).
%\end{equation}
%That is, if $\xi$ is sparse in the sense that $\|\xi\|_0\lesssim \kt^2$, it is possible to construct adaptive confidence interval. The confidence interval ${\rm CI}_{L}$ defined in \eqref{eq: linear CI} achieves this optimal rate adaptively.
%
%However, as long as $\|\xi\|_0=p^{\gamma_q}$ for some constant $\gamma_q>2\gamma$, we have
%\begin{equation}
%{\mathbf L}_{\alpha}^{*}\left(\Theta(\kt), \xi\right)\ll {\mathbf L}_{\alpha}^{*}\left(\Theta(\kt), \Theta(\ku),\xi\right).
%\end{equation}
%That is, if $\|\xi\|_0=p^{\gamma_q}$ for some constant $\gamma_q>2\gamma$, it is impossible to construct adaptive confidence intervals.
%\end{Remark}



